Dark Matter Limits From Dwarf Spheroidal Galaxies with The HAWC Gamma-Ray Observatory

The High Altitude Water Cherenkov (HAWC) gamma-ray observatory is a wide field of view observatory sensitive to 500 GeV - 100 TeV gamma rays and cosmic rays. It can also perform diverse indirect searches for dark matter (DM) annihilation and decay. Among the most promising targets for the indirect detection of dark matter are dwarf spheroidal galaxies. These objects are expected to have few astrophysical sources of gamma rays but high dark matter content, making them ideal candidates for an indirect dark matter detection with gamma rays. Here we present individual limits on the annihilation cross section and decay lifetime for 15 dwarf spheroidal galaxies within the HAWC field-of-view, as well as their combined limit. These are the first limits on the annihilation cross section and decay lifetime using data collected with HAWC.

==> Discussion.tex <==

\section{Discussion}

This analysis presented, we searched for dark matter annihilation and decay signals from fifteen dwarf spheroidal galaxies. We observed no significant excess from these sources. Thus, we calculated individual limits for fifteen dwarf spheroidal galaxies within the HAWC field-of-view using a likelihood ratio analysis method for five dark matter channels. Combined limits from a joint likelihood analysis of all dwarf spheroidal galaxies were also shown. The combined analysis was done to increase the statistical power of the analysis. These are the first limits on the dark matter annihilation cross-section and decay lifetime using data collected from the completed HAWC array. 

The HAWC combined dSph limits were also compared to four other gamma-ray experiments, Fermi-LAT, VERITAS, HESS and MAGIC. While HAWC limits with 507 days of data provide complementary results below $\sim$10 TeV, HAWC limits are the most constraining limits above 15-30 TeV. HAWC limits provide the only limits at dark matter masses higher than $\sim$20 TeV with dSphs.

We are working on improving our analysis tools for enhancing energy and angular resolution. Moreover, an approved extension of HAWC, is composed of smaller tanks around HAWC array perimeter, is being built. With more data collected, improvements on analysis tools and detector improvements, HAWC is expected to be more sensitive at lower dark matter masses, as well as improve its limits at high masses. 

In addition to the prompt gamma-ray emission discussed here for the calculations of the limits, the charged particles produced in the annihilation or decay may undergo other physical process (such as inverse Compton scattering and Brehmstruhlung) that yields more gamma rays as the charged particles propagate. The gamma-ray flux due to such phenomena peaks at lower energies that the prompt emission. Thus, the gamma-ray flux spectrum will extend down to much lower energies. For the lepton channels, particularly, this effect can increase the dark matter gamma-ray flux significantly. Inclusion of these processes may improve HAWC dark matter limits. The analysis with these additional physics processes will be conducted in the future.

\begin{acknowledgments}
  We acknowledge the support from: the US National Science Foundation (NSF);
  the US Department of Energy Office of High-Energy Physics; the Laboratory
  Directed Research and Development (LDRD) program of Los Alamos National
  Laboratory; Consejo Nacional de Ciencia y Tecnolog\'{\i}a (CONACyT), M{\'e}xico
  (grants 271051, 232656, 260378, 179588, 239762, 254964, 271737, 258865, 243290,
  132197), Laboratorio Nacional HAWC de rayos gamma; L'OREAL Fellowship for Women
  in Science 2014; Red HAWC, M{\'e}xico; DGAPA-UNAM (grants RG100414, IN111315,
  IN111716-3, IA102715, 109916, IA102917); VIEP-BUAP; PIFI 2012, 2013, PROFOCIE
  2014, 2015; the University of Wisconsin Alumni Research Foundation; the
  Institute of Geophysics, Planetary Physics, and Signatures at Los Alamos
  National Laboratory; Polish Science Centre grant DEC-2014/13/B/ST9/945;
  Coordinaci{\'o}n de la Investigaci{\'o}n Cient\'{\i}fica de la Universidad
  Michoacana. Thanks to Luciano D\'{\i}az and Eduardo Murrieta for technical
  support.
\end{acknowledgments}


